iFADIT: Invertible Face Anonymization via Disentangled Identity Transform

Face anonymization aims to conceal the visual identity of a face to safeguard the individual's privacy. Traditional methods like blurring and pixelation can largely remove identifying features, but these techniques significantly degrade image quality and are vulnerable to deep reconstruction attacks. Generative models have emerged as a promising solution for anonymizing faces while preserving a natural appearance. However, many still face limitations in visual quality and often overlook the potential to recover the original face from the anonymized version, which can be valuable in specific contexts such as image forensics. This paper proposes a novel framework named iFADIT, an acronym for Invertible Face Anonymization via Disentangled Identity Transform. The framework features a disentanglement architecture coupled with a secure flow-based model: the former decouples identity information from non-identifying attributes, while the latter transforms the decoupled identity into an anonymized version in an invertible manner controlled by a secret key. The anonymized face can then be reconstructed based on a pre-trained StyleGAN that ensures high image quality and realistic facial details. Recovery of the original face (aka de-anonymization) is possible upon the availability of the matching secret, by inverting the anonymization process based on the same set of model parameters. Furthermore, a dedicated secret-key mechanism along with a dual-phase training strategy is devised to ensure the desired properties of face anonymization. Qualitative and quantitative experiments demonstrate the superiority of the proposed approach in anonymity, reversibility, security, diversity, and interpretability over competing methods.

==> sections/0-abstract.tex <==
\begin{abstract} \label{sec:abstract}
Face anonymization aims to conceal the visual identity of a face to safeguard the individual's privacy. 
Traditional methods like blurring and pixelation can largely remove identifying features, 
but these techniques significantly degrade image quality and are vulnerable to deep reconstruction attacks. 
Generative models have emerged as a promising solution for anonymizing faces while preserving a natural appearance. 
However, many still face limitations in visual quality and often overlook the potential to recover the original face 
from the anonymized version, which can be valuable in specific contexts such as image forensics. 
This paper proposes a novel framework named iFADIT, 
an acronym for Invertible Face Anonymization via Disentangled Identity Transform.
The framework features a disentanglement architecture coupled with a secure flow-based model: 
the former decouples identity information from non-identifying attributes, 
while the latter transforms the decoupled identity into an anonymized version 
in an invertible manner controlled by a secret key. 
The anonymized face can then be reconstructed based on a pre-trained StyleGAN 
that ensures high image quality and realistic facial details. 
Recovery of the original face (aka de-anonymization) is possible upon the availability of the 
matching secret, by inverting the anonymization process based on the same set of model parameters. 
Furthermore, a dedicated secret-key mechanism along with a dual-phase training strategy 
is devised to ensure the desired properties of face anonymization. 
Qualitative and quantitative experiments demonstrate the superiority 
of the proposed approach in anonymity, reversibility, security, diversity, 
and interpretability over competing methods. 

% Face capture has become a ubiquitous activity to support various utility scenarios, 
% but has also raised global privacy concerns due to the extensive collection and 
% abuse of individuals facial data.
% including video surveillance, smart cities, smart homes, healthcare, and industrial internet.
% While, the extensive collection and abuse of personal facial data has raised 
% global concerns about individuals privacy. 
% Face anonymization aims at hiding the visual identity of a given face 
% to protect the privacy of the corresponding individual. 
% Traditional solutions to face anonymization such as blurring and pixelation 
% can erase the identity information to a large extent but these methods would seriously degrade the quality of the image 
% and are prone to deep reconstruction attacks.


% and accomplishes face 
% anonymization by transforming the decoupled identity in a secure and reversible manner. 
% To this end, a secure invertible neural network is adopted 
% to perform secure identity transformation and reconstruction. 
% A dedicated dual-phase training strategy is devised to optimize 
% the disentanglement and the transformation processes progressively. 
% Finally, qualitative and quantitative experiments demonstrate the effectiveness 
% of the proposed approach in anonymity, reversibility, security, diversity, 
% and interpretability.


% Practical solutions to face anonymization often rely on 
% simplified image obfuscations to suppress facial details, 
% but are prone to deep reconstruction attacks and identity inference by machine vision. 
% Adversarial methods effectively confound malicious face recognition systems 
% by introducing near imperceptible image perturbations, but cannot protect 
% the visual privacy of face images against human inspections. 
% With recent advancements of generative models, deep-based face anonymization 
% has emerged as a promising solution to change the identity of a face image 
% while retaining a natural facial appearance. 
% Yet, challenges remain for this type of technology, especially in 
% the anonymization diversity, reversibility, and model interpretability. 
% In this paper, we explore a disentangled methodology that decouples the 
% sensitive identity information from the image and accomplishes face 
% anonymization by transforming the decoupled identity in a secure and reversible manner. 
% To this end, a secure invertible neural network is adopted 
% to perform secure identity transformation and reconstruction. 
% A dedicated dual-phase training strategy is devised to optimize 
% the disentanglement and the transformation processes progressively. 
% Finally, qualitative and quantitative experiments demonstrate the effectiveness 
% of the proposed approach in anonymity, reversibility, security, diversity, 
% and interpretability.
\end{abstract}

\begin{IEEEkeywords}
Privacy protection, face anonymization, disentanglement, flow-based model.
\end{IEEEkeywords}

==> sections/6-biography.tex <==
% \vskip -2\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/biography/lin_yuan}}]{Lin Yuan}
received the B.Eng. degree in electronic science and technology from the University of Electronic Science and Technology of China (UESTC) in 2011 and the Ph.D. degree in electrical engineering from École Polytechnique Fédérale de Lausanne (EPFL), Switzerland in 2017. 
He is currently an associate professor of the School of Cyber Security and Information Law, Chongqing University of Posts and Telecommunications. 
His research interests include image and video analysis, multimedia privacy protection, and media forensics.
\end{IEEEbiography}


\vskip -1\baselineskip plus -1fil
\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/biography/kai_liang}}]{Kai Liang}
received the B.S. degree in electronic information engineering from the School of Electrical and Electronic Engineering, Chongqing University of Technology, Chongqing, China, in June 2021. He is currently pursuing the M.S. degree in electronic science and technology from the School of Photoelectric Engineering, Chongqing University of Posts and Telecommunications, Chongqing, China. His research interests include face privacy  protection and face editing. 
\end{IEEEbiography}


\vskip -1\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/biography/minghan_tang}}]{Minghan Tang}
is currently pursuing the B.Eng. degree in cyber security from the School of Cyber Security and Information Law, Chongqing University of Posts and Telecommunications. His research interests include information and network security, forensics, and privacy protection.
\end{IEEEbiography} 


\vskip -1\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/biography/xiao_pu}}]{Xiao Pu}
received the Ph.D. degree in electrical engineering from \'{E}cole Polytechnique F\'{e}d\'{e}rale de Lausanne (EPFL), Switzerland in 2018. 
She is currently working at the School of Cyber Security and Information Law in Chongqing University of Posts and Telecommunications.
Her research interests include cross-modal semantic understanding and natural language processing.
\end{IEEEbiography}



\vskip -1\baselineskip plus -1fil
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/biography/nannan_wang}}]{Nannan Wang}
received the B.Sc.
degree in information and computation science from
the Xi’an University of Posts and Telecommunications
in 2009 and the Ph.D. degree in information
and telecommunications engineering from Xidian
University in 2015. He is currently a Professor with
the State Key Laboratory of Integrated Services
Networks, Xidian University, Xi'an, China. He has
published over 150 articles in journals and
proceedings including IEEE T-PAMI, IJCV, CVPR and ICCV. 
His research interests include computer vision and machine learning.
\end{IEEEbiography}

\vskip -1\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{images/biography/xinbo_gao}}]{Xinbo Gao}
received the B.Eng., M.Sc., and Ph.D. degrees in signal and information processing from Xidian University, Xi'an, China, in 1994, 1997, and 1999, respectively. From 1997 to 1998, he was a Research Fellow with the Department of Computer Science, Shizuoka University, Shizuoka, Japan. From 2000 to 2001, he was a Post-Doctoral Research Fellow with the Department of Information Engineering, The Chinese University of Hong Kong, Hong Kong. Since 2001, he has been with the School of Electronic Engineering, Xidian University. He is currently a Cheung Kong Professor of Ministry of Education, a Professor of Pattern Recognition
and Intelligent System, and the president of the Chongqing University of Posts and Telecommunications. 
He is also a fellow of the IEEE and IET. His current research interests include multimedia analysis, computer vision, pattern recognition, machine learning, and wireless communications. 
He has published five books and around 200 technical articles in refereed journals and proceedings. 
%He is on the Editorial Boards of several journals, including Signal Processing (Elsevier) and Neurocomputing (Elsevier). 
%He has served as the General Chair/Co-Chair, the Program Committee Chair/Co-Chair, or a PC Member for around 30 major international conferences. 
%He is also a fellow of the Institution of Engineering and Technology. 
\end{IEEEbiography}

==> sections/formulation.tex <==
\section{Problem Formulation} \label{sec:Preliminaries of Problems Formulation}
The core of the proposed face anonymization approach
lies in transforming the identity-specific information disentangled 
from the other non-identity attributes of a given face, 
a secure and invertible manner. 
Specifically, given an input face image (noted $\bm{X}$), 
the features representing the identity information (noted $\bm{z}$) 
and non-identity attributes (noted $\bm{a}$) about that image are 
extracted separately with a {\it disentanglement} module $\mathcal{D}$:
\begin{equation}
    (\bm{z}, \bm{a}) = \mathcal{D}(\bm{X}),
\end{equation}
based on which, the original image can be reproduced by a {\it reconstruction} 
module $\mathcal{G}$ combining the two groups of features as input:
\begin{equation}
    \Tilde{\bm{X}} = \mathcal{G}\left(\bm{z}, \bm{a}\right),
    \quad \mbox{s.t. } \delta_v\left(\Tilde{\bm{X}}, \bm{X}\right) < T_v.
\end{equation}
where $\bm{\Tilde{X}}$ denotes the reconstructed image that is 
highly approximated to the original, in terms of perceptual distance signaled by metric $\delta_v$. 
Such a process is known as {\it identity disentanglement} and {\it reconstruction}, 
% , which can be formulated as:
% \begin{align}
%     \bm{z}, \bm{a}  &= E_\mathrm{id}\left(\bm{X}\right), E_\mathrm{attr}\left(\bm{X}\right), \\
%     \mbox{ s.t. } \bm{\Tilde{X}} &= G\left( M\left(\bm{z}, \bm{a}\right) \right)
% \end{align}
% \begin{equation} \label{eq:dis_rec}
%     \bm{X} = \mathcal{R}\left(\bm{z}, \bm{a}\right),
%     \quad \mbox{s.t. } (\bm{z}, \bm{a}) = \mathcal{D}(\bm{X}) 
%     % \bm{X} = \mathcal{G}\left( \mathcal{M}\left(\bm{z}, \bm{a}\right) \right), 
%     %  \quad \mbox{s.t. } 
%     %  \bm{z}, \bm{a}  = \mathcal{E}_\mathrm{id}\left(\bm{X}\right), \mathcal{E}_\mathrm{attr}\left(\bm{X}\right), 
% \end{equation}
% where $\mathcal{E}_\mathrm{id}$ and $\mathcal{E}_\mathrm{attr}$ 
% are two encoders for extracting the identity and attributes representations respectively, 
% $M$ stands for a feature fusion module and $G$ for a generative model. 


Identity disentanglement and reconstruction forms 
the base of our anonymization algorithm, which is implemented 
by transforming the original identity into a different one 
and performing reconstruction based on the transformed identity 
along with the original attributes:
\begin{equation}
    \ddot{\bm{X}} = \mathcal{R}\left(\ddot{\bm{z}}, \bm{a}\right), 
    \quad \mbox{s.t.} \quad \ddot{\bm{z}} = \mathcal{T}\left(\bm{z}, s\right),
\end{equation}
% \begin{equation}
%     \ddot{\bm{X}} = \mathcal{G}\left( \mathcal{M}\left(\ddot{\bm{z}}, \bm{a}\right) \right), 
%     \quad \mbox{s.t. } \ddot{\bm{z}} = \mathcal{T}\left(\bm{z}, s\right).
% \end{equation}
where $\ddot{\bm{X}}$ stands for the anonymized face 
and $\ddot{\bm{z}}$ for the transformed identity feature 
processed by an invertible module $T$ controlled by a secret message $s$. 
Due to the reconstructability of feature disentanglement, 
one should be able to reproduce $\ddot{\bm{z}}$ and $\bm{a}$ 
with the disentanglement module again from the anonymized face:
% $\mathcal{E}_\mathrm{id}$ and $\mathcal{E}_\mathrm{attr}$ from $\ddot{\bm{X}}$, 
% namely, performing identity disentanglement on the anonymized face again:
\begin{equation} 
    (\ddot{\bm{z}}, \bm{a}) = \mathcal{D}\left(\ddot{\bm{X}}\right),
\end{equation}
based on which, the identity of the original face can be securely generated 
by inverting $\mathcal{T}$ on $\ddot{\bm{z}}$ using the same secret $s$: 
\begin{equation}
    \check{\bm{z}} = \mathcal{T}^{-1}\left(\ddot{\bm{z}}, s\right), 
    \quad \mbox{s.t. } \delta_z\left(\check{\bm{z}}, \bm{z}\right) < T_z.
\end{equation}
where $\mathcal{T}^{-1}$ denotes a reversed process of $\mathcal{T}$ 
using the shared model parameters and $\delta$ stands for certain distance metric. 
Finally, the original image can be de-anonymized from the recovered 
facial identity and attributes relying on the same reconstruction module:
\begin{equation}
    \check{\bm{X}} = \mathcal{R}\left(\check{\bm{z}}, \bm{a}\right),
    \quad \mbox{s.t. } \delta_v\left(\check{\bm{X}}, \bm{X}\right) < T_v.
\end{equation}

In the de-anonymization phase, if any wrong secret (noted $\hat{s}$) is utilized, 
only the wrong recovery identity and recovery image will be resulted: 
% neither the recovered identity nor the recovered image would be close to their originals:
\begin{align}
    \hat{\bm{z}} = \mathcal{T}^{-1}\left(\ddot{\bm{z}}, \hat{s}\right) 
    \quad \mbox{and} \quad 
    \hat{\bm{X}} = \mathcal{R}\left(\hat{\bm{z}}, \bm{a}\right), 
\end{align}
which will be significantly different from their originals:
\begin{align}
    \delta_z\left(\hat{\bm{z}}, \bm{z}\right) \gg T_z 
    \quad \mbox{and} \quad  
    \delta_v\left(\hat{\bm{X}}, \bm{X}\right) \gg T_v.
\end{align}

In addition, different secrets would result in diverse 
anonymized appearances in terms of facial identity, 
with the attributes information remaining the same:
\begin{equation}
    \delta_v\left(\mathcal{R}\left(\mathcal{T}\left(\bm{z}, s_1\right), \bm{a}\right), \mathcal{R}\left(\mathcal{T}\left(\bm{z}, s_2\right), \bm{a}\right)\right) \gg T_v.
\end{equation}

To sum up, our anonymization approach features the following characteristics: 
\begin{itemize}
    \item \textbf{\em Anonymity:} The protected face is significantly different 
    from its original, in terms of visual perception and identity representation.
    \item \textbf{\em Utility:} Meanwhile, the anonymized image still presents 
    a natural facial appearance, keeping the same portrait pose and background, 
    and well supporting the utility of face detection. 
    \item \textbf{\em Invertibility:} The original face can be recovered from 
    the anonymized one in fidelity under certain circumstances.
    \item \textbf{\em Security:} The anonymization and de-anonymization processes 
    are guaranteed by a secret key, such that only those who possess the 
    correct key will be able to recover the original image. 
    \item \textbf{\em Interpretability:} Moreover, the core of our anonymization mechanism 
    lies in the transformation of disentangled identity information individually, 
    via an invertible neural network (INN) that exhibits enhanced interpretability 
    than conventional generative adversarial networks (GAN).  
\end{itemize}



% Next, we will describe mathematical formulas of the five characteristics in detail.

% % For the sake of clarity, we have summarized some symbols in \textcolor{red}{Tab \ref{tab:symbols}}.
% % \begin{table}
% % \caption{Notations and Meanings.}
% % \label{tab:symbols}
% % \centering
% % \renewcommand\arraystretch{2}%行间距
% % \tabcolsep=1cm %列间距
% % \begin{tabular}{|l|l|}
% % \hline
% % $\bm{X}$ & original images      \\
% % \hline
% % $\bm{\Tilde{X}}$ & inversion images      \\
% % \hline
% % $\bm{\Ddot{X}}$ & Anonymized images      \\
% % \hline
% % $\bm{\Check{X}}$ & correct recovery images      \\
% % \hline
% % $\bm{\Hat{X}}$ & wrong recovery images      \\
% % \hline
% % $\bm{\Acute{\Acute{X}}}$ & all generated images      \\
% % \hline
% % \end{tabular}
% % \end{table}

% \paragraph{\bf Anonymity}In order to anonymize the identity information of the original image, The anonymized image controlled by the key should have different information from the original image, which can be formulated as,

% \begin{equation}
%     F_{i}(T_{p}\bm{X})\ne F_{i}(\bm{X})
% \end{equation}
% where $T_{p}\bm{X}$ represents the anonymized image with the key $p$ by our anonymization method $T$. $F_{i}$ indicates for the identity of the image. 

% \paragraph{\bf Invertibility}Similarly, when the anonymized image intends to be restored, it can be restored successfully through the same key, the specific mathematical expression is as follows,

% \begin{equation}
%     T^{-1}_{p}T_{p}\bm{X}=\bm{X},
% \end{equation}
% where $T^{-1}_{p}$ denotes the inverse transformation of our anonymization method with the same key $p$.
% \paragraph{\bf Security}During the anonymization and de-anonymization phases, we aim for the generated images to possess distinct identities corresponding to different keys. This objective can be mathematically expressed as follows,

% \begin{equation}
%     F_{i}(T_{p}\bm{X})\ne F_{i}(T_{p^{\ast }}\bm{X}),
% \end{equation}
% \begin{equation}
%     F_{i}(T^{-1}_{p^{\ast }}T_{p}\bm{X})\ne F_{i}(\bm{X}).
% \end{equation}
% Thereinto, $p^\ast $ represents other keys different from key $p$. $T^{-1}_{p^{\ast }}T_{p}\bm{X}$  represents the result of deanonymization by the wrong key.

% \paragraph{\bf Utility}
% Taking into account the applicability of our framework in surveillance systems, we strive for uniform backgrounds in all images generated during the anonymization and deanonymization process. This objective can be mathematically formulated as follows,

% \begin{equation}
%     F_p(\bm{X}) = F_p(\bm{\Acute{\Acute{X}}}),
% \end{equation}

% % Among them, $\bm{\Acute{\Acute{X}}}$ represents all images generated during the anonymization and de-anonymization processes. 
% where $F_p$ denotes the perception distance.

% \paragraph{\bf Interpretability}In the previous methods, such as FIT, Riddle, etc, the whole image was mapped into the feature spectrum for anonymization and de-anonymization, and these methods often lacked the interpretability of the models. Therefore, We decouple identity and attributes separately, and achieve the effects of anonymization and deanonymization by only modifying identity information. Besides, we use an invertible neural network in the process of identity transformation, which is invertible on the mathematical logic. Therefore, This decoupled invertible network makes model more interpretable.

